A Study of Dropout-Induced Modality Bias on Robustness to Missing Video Frames for Audio-Visual Speech Recognition

Advanced Audio-Visual Speech Recognition (AVSR) systems have been observed to be sensitive to missing video frames, performing even worse than single-modality models. While applying the dropout technique to the video modality enhances robustness to missing frames, it simultaneously results in a performance loss when dealing with complete data input. In this paper, we investigate this contrasting phenomenon from the perspective of modality bias and reveal that an excessive modality bias on the audio caused by dropout is the underlying reason. Moreover, we present the Modality Bias Hypothesis (MBH) to systematically describe the relationship between modality bias and robustness against missing modality in multimodal systems. Building on these findings, we propose a novel Multimodal Distribution Approximation with Knowledge Distillation (MDA-KD) framework to reduce over-reliance on the audio modality and to maintain performance and robustness simultaneously. Finally, to address an entirely missing modality, we adopt adapters to dynamically switch decision strategies. The effectiveness of our proposed approach is evaluated and validated through a series of comprehensive experiments using the MISP2021 and MISP2022 datasets. Our code is available at https://github.com/dalision/ModalBiasAVSR

==> sec/rebuttal.tex <==
\clearpage
\setcounter{page}{1}
% \maketitlesupplementary


\crefname{section}{Sec.}{Secs.}
\Crefname{section}{Section}{Sections}
\Crefname{table}{Table}{Tables}
\crefname{table}{Tab.}{Tabs.}

\newcommand{\toreviewer}[1]{\vspace{0.0em}\noindent \textcolor{blue}{\textbf{#1 \hspace{0.2em}}}}
\newcommand{\issue}[1]{\vspace{0.1em}\noindent \textcolor{blue}{\textbf{#1 \hspace{0.2em}}}}



\def\PaperID{17309} % *** Enter the CVPR Paper ID here
\def\confName{CVPR}
\def\confYear{2024}
\setlength{\abovecaptionskip}{0pt}
\setlength{\textfloatsep}{0pt}
\setlength{\intextsep}{0pt}

% \maketitle

\thispagestyle{empty}
\appendix
% Thanks to all the reviewers and chairs for the time and constructive feedback. We address comments as follows.
We appreciate all reviewers for acknowledging the contribution of this work and the quality of the presentation. We will address the improvements and clarifications as follows.

\issue{More discussion on literature review ($@$R1)} 
Thanks a lot for recognizing the versatility of our method. We have rewritten the literature review section and discussed more related tasks, focusing on the problem of modality missing, including sensor robustness in autonomous driving, multimodal sentiment analysis and visual question answering.

\issue{Additional experiments with low-SNR audio and more datasets ($@$R2\&R3)}
In this work, all the experiments are evaluated in real-world home TV scenarios with far-field audios (around 0 to -5 dB SNR) containing high-level noise from other speakers and TV background noise (lines 404-410). In Table \ref{table:zero-shot}, we further analyze our methods with quantified noisy audio using near-field audio (much cleaner than far-field audio) and zero-shot Babble noise from NOISEX where the system symbol is the same as in Table \ref{table2:drpout comparison}. As a result, the proposed AV6 is more robust to noise interference, especially for zero-shot noise, compared to the excessively modality-biased model AV1 and A0. For more evaluation, in Table \ref{table:LRS}, we compare our system with widely used dropout methods (lines 502-510) on LRS3 \cite{afouras2018lrs3}, under different SNR conditions with zero-shot Pink noise from NOISEX. As a result, our method shows a clear performance advantage with audio-visual and audio-only input. 


\issue{Marginal improvements ($@$R3)} 
Our goal for an ideal video missing robustness method is to concurrently maintain both performance and robustness. It is expected to (a) enhance robustness without performance degradation on complete input and (b) match the quality of the audio-only model when tested with audio-only input. In Table 6, when compared to a model trained on a large video dropout rate (e.g. 0.5 in AV1) with audio-only input, our proposed method AV6 shows significant performance improvement (25.91 vs 24.94) and successfully matches the quality of the audio-only model when tested with audio-only input A0 (24.94 vs 25.13) as highlighted by R1. More importantly, when compared with AV1, our key contribution lies in simultaneously preventing performance degradation with complete input  (23.26 vs 21.11). However, investigating ways to enhance audio-only testing performance by leveraging visual input during training is an intriguing avenue for future, and we intend to delve deeper into this research.





\issue{Modality imbalance issue in teacher model ($@$R3)} 
Without considering video missing, the modality imbalance issue (e.g. semantic info, quality) has already been addressed in prior work \cite{Dai2023icme}. Our teacher model follows their training pipeline (line 411), retaining a modality-biased nature, yet achieving optimal parameters with complete input. Two-stage decoupled training and audio data augmentation (line 904, Appendix) are employed to ensure this. We clarify that we never attempt to eliminate modality bias entirely, as it is not always harmful. It is wiser to match different missing inputs with their respective optimized modality bias pattern (activating MS-adapter for server video missing input) or guide slightly incomplete input to align with a complete data pair in the latent space (guided by MDA-KD).

\issue{Similar to AV-HuBERT ($@$R3)} 
We clarify that the mask prediction-based self-supervised method used in AV-HuBERT \cite{9:shi2022learning} might cause the confusion, which is optimized by classifying the discrete tokens extracted through offline k-means clustering. However, it differs from MDA-KD, which is optimized by the online latent distribution approximation in the form of knowledge distillation.


\issue{Tiny performance gap between training dropout rate 0.3\&0.5 on test dropout rate 0.0\&1.0 ($@$R3)}
 In Figure \ref{fig1:CER_Droprate}, we compare the overall tendency of  CER curves of different AVSR models trained on various video training dropout rates, indicating varying degrees of modality bias on audio. The comparison aims to illustrate two key points: (1) the influence of increasing dropout-induced bias on CER curves, serving as a prelude of dropout-induced modality bias (2) an intuitive description of the dilemma problem in common dropout techniques (lines 61-66). Two overall tendencies could be observed to achieve above objectives. (a) With an increasing training dropout rate, the CER curve gradually shifts from an ascending curve (red line) to a horizontal parallel line (dotted line). (b) The model trained with a higher dropout rate deteriorates more with complete or slightly missing input but performs better on severely missing input. To address the reviewer's confusion, we clarify that the tiny gap in performance indicates that modality bias does not linearly shift with the training dropout rate at these specific test dropout rates. Figure \ref{fig2:Relative-CER_Droprate} shows that it resembles a reversed tan function curve. However, whether linear or non-linear, the overall trend (a) (b) remains unchanged. 


 \captionsetup[table]{belowskip=-10pt}
\begin{table}[!t]
\fontsize{7}{8}\selectfont
\resizebox{1.10\columnwidth}{!}{
\begin{tabular}{cccccc}\toprule[0.7pt]
\multirow{2}{*}{\textbf{Models}} & \multirow{2}{*}{\textbf{Near Field}} & \multirow{2}{*}{\textbf{Far Field}} & \multicolumn{3}{c}{\textbf{Zero-shot Babble Noise}} \\ \cline{4-6} 
                                 &                                      &                                     & 0dB             & -2.5dB           & -5dB           \\ \hline
A0                               & 18.10                                & 25.13                               & 33.52           & 62.17            & 75.76          \\
AV1                              & 17.71                                & 23.26                               & 29.40           & 51.63            & 63.80          \\
AV6                              & \textbf{16.86}                       & \textbf{21.11}                      & \textbf{26.67}  & \textbf{44.97}   & \textbf{55.65} \\ \bottomrule[0.7pt]
\end{tabular}}
\caption{System comparison with low-SNR audio input.}
\label{table:zero-shot}
\end{table}

\captionsetup[table]{belowskip=0pt}
\begin{table}[!t]
{\fontsize{15}{17}\selectfont
\resizebox{1.10\columnwidth}{!}{
\begin{tabular}{ccccccccc}
\toprule[1.7pt]
\multirow{2}{*}{\textbf{Dataset}} & \multirow{2}{*}{\textbf{Method}} & \multicolumn{3}{c}{\textbf{AV}}                &  & \multicolumn{3}{c}{\textbf{AO}}                  \\ \cline{3-5} \cline{7-9} 
                                  &                                  & 0dB           & -2.5dB        & -5dB           &  & 0dB            & -2.5dB         & -5dB           \\ \hline
\multirow{4}{*}{LRS3}             & Cascade Utt                      & 6.29          & 12.91         & 20.34          &  & 13.32          & 27.47          & 43.55          \\
                                  & Dropout Utt                      & 4.06          & 6.39          & 10.76          &  & 11.19          & 22.18          & 37.63          \\
                                  & AV Dropout Utt                   & 4.24          & 6.84          & 11.15          &  & 10.68          & 22.19          & 36.66          \\
                                  & Ours                             & \textbf{3.27} & \textbf{5.79} & \textbf{8.80}  &  & \textbf{8.00}  & \textbf{18.72} & \textbf{31.45} \\ 
\bottomrule[1.7pt]
\end{tabular}}}
\caption{System comparison on LRS3.}
\label{table:LRS}
\end{table} 

\issue{Additional response ($@$R3)}
We appreciate the detailed and constructive comments from R3, providing a distinct perspective to revisit this work and assisting us in further enhancing its quality. We truly hope our response could clarify the confusion and we look forward to the reviewer considering an improvement in the score, taking into account paper's contributions and other reviewers' comments.
